Quantifying the Blockchain Trilemma: A Comparative Analysis of Algorand, Ethereum 2.0, and Beyond

Blockchain technology is essential for the digital economy and metaverse, supporting applications from decentralized finance to virtual assets. However, its potential is constrained by the "Blockchain Trilemma," which necessitates balancing decentralization, security, and scalability. This study evaluates and compares two leading proof-of-stake (PoS) systems, Algorand and Ethereum 2.0, against these critical metrics. Our research interprets existing indices to measure decentralization, evaluates scalability through transactional data, and assesses security by identifying potential vulnerabilities. Utilizing real-world data, we analyze each platform's strategies in a structured manner to understand their effectiveness in addressing trilemma challenges. The findings highlight each platform's strengths and propose general methodologies for evaluating key blockchain characteristics applicable to other systems. This research advances the understanding of blockchain technologies and their implications for the future digital economy. Data and code are available on GitHub as open source.

==> tabs/tab4.tex <==
\definecolor{col1}{RGB}{229,243,255} % 更浅的蓝色
\definecolor{col2}{RGB}{204,229,255}
\definecolor{col3}{RGB}{179,217,255}
\definecolor{col4}{RGB}{153,204,255}
\definecolor{col5}{RGB}{128,191,255}
\definecolor{col6}{RGB}{102,178,255}
\definecolor{col7}{RGB}{77,166,255}
\definecolor{col8}{RGB}{51,153,255} 


\begin{table*}
\centering
\caption{ On-chain data for Algorand from January 2019 to September 2023 via BitQuery’s open APIs, and for Ethereum 2.0 from June 2019 to September 2023 through Beacon Explorer using the SPIDER framework.}
\label{table:4}
\begin{tabularx}{\textwidth}{
    >{\columncolor{col1}}p{1.2cm} 
    >{\columncolor{col2}}p{1.9cm}
    >{\columncolor{col3}}p{2cm} 
    >{\columncolor{col4}}p{0.35cm} 
    >{\columncolor{col5}}p{0.7cm} 
    >{\columncolor{col6}}p{1.1cm} 
    >{\columncolor{col7}\color{black}}p{2.9cm} 
    >{\columncolor{col8}\color{black}}p{4.6cm}
}
\toprule
\textbf{Data Type} & \textbf{Data Frame} & \textbf{Description} & \textbf{Unit} & \textbf{Type} & \textbf{Frequency} & \textbf{Range} & \textbf{File Name} \\ 
\midrule
Block & Daily Block Count & Numbers of blocks produced per day & NA & Integer & Daily & 0\textasciitilde{}7180 & daily\_block\_count.csv \\
 & Average Block Time & Average consensus time per block & S & Float & Daily & 4.46\textasciitilde{}30.57 & avg\_blk\_time.csv \\
 & Average Gas Used by Blocks & Average gas used per block & NA & Float & Daily Sum & 0\textasciitilde{}15511762.25 & gas\_used\_avg\_by\_blk.csv \\
Transaction & Transaction Count & Transaction count per day & NA & Integer & Daily & 0\textasciitilde{}1932226 & daily\_transactions.csv \\
 & Gas Limit & Gas limit amount per day & Eth & Integer & Daily Sum & 5000\textasciitilde{}30076713.92 & gas\_limit.csv \\
 & Burned Fees & Used tokens for transactions per day & Eth & Float & Daily & 0\textasciitilde{}71718.88 & burned\_fees.csv \\
Account & Validator Count & Validator counts per day & NA & Integer & Daily & 21063\textasciitilde{}771738 & validator\_data.csv \\
 & Average Validator Balance & Average account balance of validators per day & Eth & Float & Daily & 32.00953203\textasciitilde{}34.00950871 & validator\_avg\_balance.csv \\
 & Participation Rate & Overall participation rate per day & NA & Float & Daily(\%) & 0.941524213\textasciitilde{}0.99728444 & participation\_rate.csv \\
Network & Network Liveness & Block count for confirmation & NA & Integer & Daily & 2\textasciitilde{}12 & network\_Liveness.csv \\
Block & Block Info & Block timestamp, address, height & NA & String & Daily & NA & al\_block\_data.csv \\
 & Proposer Count & Proposer count per day & NA & Integer & Daily & 31\textasciitilde{}130 & al\_block\_data\_proposercount\_reward.csv \\
Transaction & Transaction Count & Transaction count per day & NA & Float & Daily & 913\textasciitilde{}9271981 & al\_transac\_data\_count\_fee.csv \\
 & Burned Fees & Tokens used for transactions & Algo & Float & Daily & 1.47588\textasciitilde{}33113.44687 & al\_transac\_data\_count\_fee.csv \\
Account & Block Reward & Reward for block proposal per day & Algo & Float & Daily & 141.059024\textasciitilde{}5184.994864 & al\_block\_data\_reward.csv \\
Contract & Contract Calls & Overall contract calls per day & NA & Integer & Daily & 1\textasciitilde{}197459 & al\_contracts\_calls\_unique\_calls.csv \\
 & Unique Calls & Unique contract calls & NA & Integer & Daily & 1\textasciitilde{}10149 & al\_contracts\_calls\_unique\_calls.csv \\
\bottomrule
\end{tabularx}
\end{table*}
